Optimizing Photonic Nanostructures via Multi-fidelity Gaussian Processes

We apply numerical methods in combination with finite-difference-time-domain (FDTD) simulations to optimize transmission properties of plasmonic mirror color filters using a multi-objective figure of merit over a five-dimensional parameter space by utilizing novel multi-fidelity Gaussian processes approach. We compare these results with conventional derivative-free global search algorithms, such as (single-fidelity) Gaussian Processes optimization scheme, and Particle Swarm Optimization---a commonly used method in nanophotonics community, which is implemented in Lumerical commercial photonics software. We demonstrate the performance of various numerical optimization approaches on several pre-collected real-world datasets and show that by properly trading off expensive information sources with cheap simulations, one can more effectively optimize the transmission properties with a fixed budget.

==> method-mfmigreedy.tex <==
\section{The Multi-fidelity BO Framework}
\label{sec:alg}
We now present \algname, a general framework for multi-fidelity Gaussian process optimization. In a nutshell, \algname attempts to balance the ``explorative'' low-fidelity actions and the more expensive target fidelity actions, based on how much information (per unit cost) these actions could provide about the overall optimization problem. % To keep it
Concretely, \algname proceeds in rounds under a given budget $\budget$. Each round can be divided into two phases: (i) an exploration (i.e., information gathering) phase, where the algorithm focuses on exploring the low fidelity actions, and (ii) an optimization phase, where the algorithm tries to optimize the payoff function $\tarf$ by performing an action $\action{\ex, \targetfid}$ at the target fidelity. The pseudo-code of the algorithm is provided in \algref{alg:main}.
% The algorithm is presented in \algref{alg:main}. \figref{fig:alg:illustration} illustrate \algref{alg:main} in two different iterations.

\begin{algorithm}[t]
  \nl {\bf Input}: {Total budget $\budget$; cost $\costof{i}$ for all fidelities $i \in [\targetfid]$}; joint GP (prior) distribution on $\{\fidelity_i, \noise_i\}_{i\in[\targetfid]}$\\ % between $\fidelity_i$ and noise $$. \\
  \Begin{
    % \nl $\alpha = \frac{\max_\ex \infgain{\action{\ex, \targetfid}}}{\sqrt{\budget} \costof{\targetfid}} $ \\
    \nl $\selected \leftarrow \emptyset$ \\
    \nl $B \leftarrow \budget$ \tcc*{initialize remainig budget}
    \While{$B > 0$} % outer loop
    {
      \tcc{explore with low fidelity}
      \nl $\eplow \leftarrow$ \explorelf $\paren{B, [\costof{\fid}], \GP{\{\utility_\fid, \noise_\fid\}_{\fid\in[\targetfid]}}, \selected}$ \\
      \tcc{select target fidelity}
      \nl $\ex^* \leftarrow \sfgpopt(\GP{\{\tarf, \noise_\targetfid\}}, \bobs_{\selected \cup \eplow})$ \label{ln:alg:main:sfgpout}\\
      \nl $\selected \leftarrow \selected \cup \eplow \cup \{\action{\ex^*,\targetfid}\}$\\
      \nl $B \leftarrow \budget - \Cost_\selected$ \tcc*{update remaining budget}
    }
    \nl {\bf Output}: Optimizer of the target function $\tarf$ \\
  }
  \caption{Multi-fidelity Most Infomative Greedy Optimization (\algname)}\label{alg:main}
\end{algorithm}

\paragraph{Exploration phase}
% As is the case for online learning problems in general,
A key challenge in designing the algorithm is to decide when to stop exploration (or equivalently, to invoke the optimization phase). Note that this is analogous to the exploration-exploitation dilemma in the classical single-fidelity Bayesian optimization problems; the difference is that in the multi-fidelity setting, we have a more distinctive notion of ``exploration'', and a more complicated structure of the action space (i.e., each exploration phase corresponds to picking a set of low fidelity actions). Furthermore, note that there is no explicit measurement of the relative ``quality'' of a low fidelity action, as they all have uniform reward by our modeling assumption (c.f. Eq.~\eqref{eq:reward}); hence we need to design a proper heuristic to keep track of the progress of exploration.

We consider an information-theoretic selection criterion for picking low fidelity actions. The quality of a low fidelity action $\action{\ex, \fid}$ is captured by the \emph{information gain}, defined as the amount of entropy reduction in the posterior distribution of the target payoff function\footnote{An alternative, more aggressive information measurement is the information gain over the \emph{optimizer} of the target function $\tarf$ \citep{hennig2012entropy}, i.e., $\mathbb{I}\parencond*{\obs_{\action{\ex,\fid}}; \argmax_{\ex}\tarf(\ex)}{\bobs_\selected}$, or the \emph{optimal value} of $\tarf$ \citep{wang2017max}, i.e., $\mathbb{I}\parencond*{\obs_{\action{\ex,\fid}}; \max_{\ex}\tarf(\ex)}{\bobs_\selected}$.
  % Since we cannot directly measure the benefit of low fidelity
  % There are different of measurements
}: $\condinfgain{\obs_{\action{\ex, \fid}} }{\bobs_\selected} = \condentropy{\obs_{\action{\ex, \fid}} }{\bobs_\selected} - \condentropy{\obs_{\action{\ex, \fid}} }{\tarf, \bobs_\selected}$. Here, $\selected$ denotes the set of previously selected actions, and $\bobs_{\selected}$ denote the observation history. % Since the overall optimization problem is under a budget constraint $\budget$,
Given an exploration budget $B$, our objective for a single exploration phase is to find a set of low-fidelity actions, which are (i) maximally informative about the target function, (ii) better than the best action on the target fidelity when considering the information gain per unit cost (otherwise, one would rather pick the target fidelity action to trade off exploration and exploitation), and (iii) not overly aggressive in terms of exploration (since we would also like to reserve a certain budget for performing target fidelity actions to gain reward).

Finding the optimal set of actions satisfying the above design principles is computationally prohibitive, as it requires us to search through a combinatorial (for finite domain) or even infinite (for continuous domain) space. In \algref{alg:explorelf}, we introduce \explorelf, a key subroutine of \algname, for efficient exploration on low fidelities. At each step, \explorelf takes a greedy step w.r.t. the benefit cost ratio over all actions. To ensure that the algorithm does not  explore excessively, we consider the following stopping conditions: (i) when the budget is exhausted (\lnref{alg:explorelf:ln:budget}), (ii) when a single target fidelity action is better than all the low fidelity actions in terms of the benefit cost ratio (\lnref{alg:explorelf:ln:targetcheck}), and (iii) when the cumulative benefit cost ratio is small (\lnref{alg:explorelf:ln:infgaincheck}). Here, the parameter $\beta$ is set to be  $\bigOmega{\frac{1}{\sqrt{B}}}$ to ensure low regret, and we defer to detailed discussion of the choice of $\beta$ to \secref{sec:analysis:regret}.

% As we can see from \algref{alg:explorelf}, as the
% Our exploration strategy, \explorelf, is described \algref{alg:explorelf}.
\begin{algorithm}[t]
  \nl {\bf Input}: {Exploration budget $B$; cost $[\costof{\fid}]_{\fid \in [\targetfid]}$; joint GP distribution on $\{\fidelity_i, \noise_i\}_{i\in[\targetfid]}$; previously selected items $\selected$}\\ % between $\fidelity_i$ and noise $$ \\
  \Begin{
    \nl $\eplow \leftarrow \emptyset$ \tcc*{selected actions}
    \nl $\Cost_\eplow \leftarrow 0$ \tcc*{cost of selected actions}
    % \nl $\beta \leftarrow \bigO{\frac{1}{\sqrt{B}}}$ \tcc*{stopping condition}
    \nl $\beta \leftarrow \frac{1}{\alpha(B)}$ \tcc*{threshold (c.f. \thmref{thm:general:datadependent-bound})}
    % \tcc{explore with lower fidelities}
    \While{true}
    {
      \tcc{greedy benefit-cost ratio}
      \nl $\action{\ex^*, \fid^*} \leftarrow
      \argmax_{\action{\ex, \fid}: \costof{\fid} \leq B-\Cost_\eplow - \costof{\targetfid}} \frac{\condinfgain{\obs_{\action{\ex, \fid}}}{\bobs_{\selected \cup \eplow}}}{\costof{\fid}}$ \\
      % \If{$\fid^*\neq \targetfid$} % stopping condition
      % {
      \If{$\fid^* = \nan$}
      {
        \nl break \label{alg:explorelf:ln:budget}
        \tcc*{budget exhausted}
      }
      \If{$\fid^* = \targetfid$}
      {
        \nl break \label{alg:explorelf:ln:targetcheck}
        \tcc*{worse than target}
      }
      \ElseIf{ $\frac{\condinfgain{\bobs_{\eplow \cup \{ \action{\ex^*, \fid^*} \} } }{\bobs_\selected}} {\paren{\Cost_\eplow + \costof{\fid^*}}} < \beta$}
      {
        \nl \label{alg:explorelf:ln:infgaincheck} break \tcc*{low cumulative ratio}
      }
      \Else
      {
        \nl $\eplow \leftarrow \eplow \cup \{\action{\ex^*,\fid^*}\}$ \\
        \nl $\Cost_\eplow \leftarrow \Cost_\eplow + \costof{\fid^*}$
      }
    }
  }
  \nl {\bf Output}: Selected set of items $\eplow$ from lower fidelities \\
  \caption{\explorelf: Explore low fidelities}\label{alg:explorelf}
\end{algorithm}

\paragraph{Optimization phase} At the end of the exploration phase, \algname updates the posterior distribution of the joint GP using the full observation history, % From the updated posterior, \algname
and searches for a target fidelity action via the (single-fidelity) GP optimization subroutine \sfgpopt (\lnref{ln:alg:main:sfgpout}). % Here, \sfgpopt implements the (single-fidelity) GP optimization algorithm only on the target fidelity. The subroutine \explorelf is detalied in algorithm \algref{alg:explorelf}.
Here, \sfgpopt could be \emph{any} off-the-shelf Bayesian optimization algorithm, such as \sfgpucb \citep{srinivas10gaussian}, \sfgpmi \citep{contal2014gaussian}, \sfest \citep{wang2016optimization} and \sfmves \citep{wang2017max}, etc. Different from the previous exploration phase which seeks the an informative set of low fidelity actions, the GP optimization subroutine aims to trade off exploration and exploitation on the target fidelity, and outputs a single action at each round. %
\algname then proceeds to the next round until it exhausts the preset budget, and eventually outputs an estimator of the target function optimizer.

% \begin{figure}[t]
%   \centering
%   \includegraphics[trim={0pt 0pt 0pt 0pt}, width=.48\textwidth]{./fig/empty.png}
%   \includegraphics[trim={0pt 0pt 0pt 0pt}, width=.48\textwidth]{./fig/empty.png}
%   \caption{Illustration of the algorithm}
%   \label{fig:alg:illustration}
% \end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

